Image Inpainting Based On Coherence Transport With Adapted Distance Functions

We discuss an extension of our method Image Inpainting Based on Coherence Transport. For the latter method the pixels of the inpainting domain have to be serialized into an ordered list. Up till now, to induce the serialization we have used the distance to boundary map. But there are inpainting problems where the distance to boundary serialization causes unsatisfactory inpainting results. In the present work we demonstrate cases where we can resolve the difficulties by employing other distance functions which better suit the problem at hand.

==> macros.tex <==
%%
% at "@" und "!" als letter
%% 
\expandafter\edef\csname @catcode\endcsname{\the\catcode`\@}
\expandafter\edef\csname !catcode\endcsname{\the\catcode`\!}
\catcode`\@11
\catcode`\!11

%%%% skips
\smallskipamount=3pt plus 0.5pt minus 0.5pt
\medskipamount=6pt plus 1pt minus 1pt
\bigskipamount=12pt plus 2pt minus 2pt

%%% Tabellen
\renewcommand{\arraystretch}{1.5}

%%% Mengen
\def\A{{\mathcal{A}}}                 %% generische sigma-Algebra
\def\B{{\mathcal{B}}}                 %% Borel-sigma-Algebra
\def\Sk{{\mathcal{S}}} 		%% Skelett
\def\N{{\mathbb{N}}}                  %% natürliche Zahlen
\def\Z{{\mathbb{Z}}}                  %% ganze Zahlen
\def\R{{\mathbb{R}}}                  %% reellen Zahlen
\def\1{{\mathbb{1}}}			%% charakteristische Funktion
\def\Rinfty{\overline{\mathbb{R}} }         %% reellen Zahlen mit +infty und -infty


% meine Funktionenmengen
\def\FD{{\mathcal{F}}}                %% Functional domain general
\def\FR{{\mathcal{G}}}                %% Functional range general
\def\FF{{\mathfrak{F}}}                 %% Functional domain in L^1
\def\FX{{\mathfrak{X}}}                %%  Functional domain in BV
\def\FB{{\mathfrak{B}}}                %%  Randfunktionen aus BV  
                

%%% Parameter
\def\const{{\mathrm{const}}}          %% irgendeine Konstance

%%% Funktionenräume 
\def\C{C}                                      %% stetige Funktionen
\def\L{L}                                         %% Lebesgue intbare Funktionen
\def\Lloc{L_{\mathrm{loc}}}           %% lokal Lebesgue intbare Funktionen
\def\W{W}                                          %% Sobolev Raum
\def\BV{{\mathit{BV}}}                %% Funktionen beschr. Variation
\def\SBV{{\mathit{SBV}}}              %% spez. Funktionen beschr. Variation
\def\PT{{\mathit{P}}}                %% periodische Testfunktionen

%%% Maße
\def\Hm{{\mathcal{H}}}                %% Hausdorff-Maß
\def\Lm{{\mathcal{L}}}                %% Lebesgue-Maß
\def\Mloc{{\mathcal{M}_{\mathrm{loc}}}}%% vektorwertige Radon-Maße
\def\M{{\mathcal{M}}}                 %% endliche Radon-Maße

%% Verweis auf Gleichung
\def\refEq#1{(\ref{#1})}

%% Intervall
\def\IV#1#2,#3#4{\left#1#2,#3\right#4}
\def\usIV#1#2;#3#4{\mathopen{#1}#2;#3\mathclose{#4}}

%% Skalarprodukt / Norm
\def\SP#1#2,#3#4{\left#1#2,#3\right#4}
\def\Norm#1#2{\Vert#1\Vert_{#2}}                                   %% Norm
\def\sNorm#1#2{\left\Vert#1\right\Vert_{#2}}                 %% sNorm: norm mit left und right Skalierung
\def\genNorm#1{\Vert#1\Vert}                                          %% generische Norm

%% Operatoren
\def\arclength{\mathop{\operator@font arclength}}                       %% Bogenlänge
\let\bd\partial                                                                                          %% Rand, boundary
\let\pd\partial                                                                                          %% partial derivative
\let\cl\overline                                                                                         %% Abschluss closure
\def\div{\mathop{\operator@font div}}                                             %% Divergenz
\DeclareMathOperator{\dist}{dist}                              %% distance
\def\liminf{\mathop{\smash{\operator@font lim\,inf}}}        % liminf
\def\limsup{\mathop{\smash{\operator@font lim\,sup}}}        % limsup
\def\supp{\mathop{\smash{\operator@font supp}}}          % support
\def\O{\mathcal{O}}                                          % Landau
\def\o{{o}}                                                          % Landau klein
\def\Var{\mathop{\operator@font Var}}                        % Variation
\def\trace{\mathop{\operator@font trace}}                        % spur
\DeclareMathOperator{\sgn}{sgn}                                % signum
\DeclareMathOperator{\lingen}{span}                                % span
\def\inner#1{\mathring{#1}} 
\def\diam{\mathop{\operator@font diam}}                         %% Diameter

%%% binäre Operatoren
\def\longrightharpoonup{%                                    % long-Variante von rightharpoonup
  \relbar\joinrel\rightharpoonup
}
\let\wo\backslash                                            %% ohne
\let\nb\sim                                                  %% Nachbarschaft
\def\rto{\,\hbox{\vrule height7pt width0.5pt depth0pt        %% Restriktion
  \vrule height0.5pt width5pt depth0pt}\,}
\def\cc{\mathbin{\mathord{\subset}\!\mathord{\subset}}}        %% compact subset
\let\asymp\sim                                               %% asymptot. Verh.
\def\symdiff{\mathbin{\Delta}}                               %% symmetr. Diff.
\let\gdw\Leftrightarrow                                      %% genau dann wenn
\def\strongto{%                                              %% starke Konvergenz
  \@ifnextchar[\@strongto{\@strongto[]}}
\def\@strongto[#1]{%
  \def\temp{#1}%
  \ifx\temp\empty
  \to
  \else
  \mathrel{\mathop{\longrightarrow}\limits_{\scriptstyle#1}}%
  \fi
}
\def\weakto{%                                                % schwache Konvergenz
  \@ifnextchar[\@weakto{\@weakto[]}}
\def\@weakto[#1]{%
  \def\temp{#1}%
  \ifx\temp\empty
  \rightharpoonup
  \else
  \mathrel{\mathop{\longrightharpoonup}\limits_{\scriptstyle#1}}%
  \fi
}
\def\weaksto{%                                                % schwache* Konvergenz
  \@ifnextchar[\@weaksto{\@weaksto[]}}
\def\@weaksto[#1]{%
  \def\temp{#1}%
  \ifx\temp\empty
  \mathrel{\mathop{\rightharpoonup}\limits^{\scriptstyle*}}%
  \else
  \mathrel{\mathop{\longrightharpoonup}\limits^{\scriptstyle*}_{\scriptstyle#1}}%
  \fi
}
\let\symdiff\Delta                                            % symmetrische Differenz
\def\dotarg{\mathord{\, .\,}}                              % beliebiges Argument mit Punkt


%%
% Theoreme und Environments
%%


\newtheorem{theo}{Theorem}[section]
\newtheorem{lem}[theo]{Lemma}%[chapter]
\newtheorem{cor}[theo]{Corollary}%[chapter]
\newtheorem{prop}[theo]{Proposition}%[chapter]
\newtheorem{defi}[theo]{Definition}%[chapter]
\newtheorem{req}[theo]{Requirement}%[chapter]
\newtheorem{prob}[theo]{Problem}%[chapter]
\newtheorem{rem}[theo]{Remark}%[chapter]

%% Beweis:
%% Umbruch danach nicht unerwünscht
%\let\orig@end@proof\endproof
%\def\endproof{\orig@end@proof\penalty-500\relax}

%% Davor hat auch niemand was dagegen
%\let\orig@proof\proof
%\def\proof{\penalty-500 \orig@proof}


%% kein Absatz Einzug
%\parindent=0pt

%% dafür aber etwas Parskip zur Abtrennung verschiedener Absätze
%\parskip=3pt plus1.5pt minus1pt

%% die Ränder
\evensidemargin=2cm %54pt
\oddsidemargin=2cm %54pt

%\advance\evensidemargin -2.5mm
%\advance\oddsidemargin -2.5mm

%% marks für Headline
%\def\chaptermark#1{%
%  \markboth {%
%    \ifnum \c@secnumdepth >\m@ne
%      \if@mainmatter
%        \@chapapp\ \thechapter\enskip%
%      \fi
%    \fi
%    #1}{}}%
%\def\sectionmark#1{%
%  \markright {%
%    \ifnum \c@secnumdepth >\z@
%      \thesection\enskip%
%    \fi
%    #1}}

\endinput

